Online Laplace Model Selection Revisited

The Laplace approximation provides a closed-form model selection objective for neural networks (NN). Online variants, which optimise NN parameters jointly with hyperparameters, like weight decay strength, have seen renewed interest in the Bayesian deep learning community. However, these methods violate Laplace's method's critical assumption that the approximation is performed around a mode of the loss, calling into question their soundness. This work re-derives online Laplace methods, showing them to target a variational bound on a mode-corrected variant of the Laplace evidence which does not make stationarity assumptions. Online Laplace and its mode-corrected counterpart share stationary points where 1. the NN parameters are a maximum a posteriori, satisfying the Laplace method's assumption, and 2. the hyperparameters maximise the Laplace evidence, motivating online methods. We demonstrate that these optima are roughly attained in practise by online algorithms using full-batch gradient descent on UCI regression datasets. The optimised hyperparameters prevent overfitting and outperform validation-based early stopping.

==> algorithms/algo_online_laplace.tex <==
\begin{algorithm2e}[H]
	\SetAlgoLined
	\DontPrintSemicolon
	\KwData{Neural network $f$, Observation $x$,  Linearisation point $\tilde \theta$, Weights to optimise $v$, Likelihood function $\ell(\cdot, y)$, Machine precision $\epsilon$}
	$\delta \gets \sqrt{\epsilon} (1+\norm{\tilde \theta}_{\infty}) / \norm{v}_{\infty}$ \tcp*{Set FD stepsize \citep{ANDREI2009Accelerated}}
	$\hat{y} = J(x) \cdot v   \approx \frac{f(x, \tilde \theta + \delta v ) - f(x, \tilde \theta - \delta v ) }{2 \delta}$ \tcp*{Two sided FD approximation to Jvp}
	$g = \partial_{\hat{y}} [\ell(\hat{y}, y)](J(x)\cdot v)$ \tcp*{Evaluate gradient of loss at $J(x) \cdot v$ }
	$g^{T} \cdot J(x) = \partial_{\theta} [g^{T} \cdot f(\theta, x)](\tilde \theta) $ \tcp*{Project gradient with backward mode AD}
\KwResult{$g^{T} \cdot J(x)$}
\caption{Efficient evaluation of the likelihood gradient for the linearised model}
\label{alg:linear_MAP_algorithm}
\end{algorithm2e}


